Collisional Cooling of Ultracold Molecules

Since the original work on Bose-Einstein condensation, quantum degenerate gases of atoms have allowed the quantum emulation of important systems from condensed matter and nuclear physics, as well as the study of novel many-body states with no analog in other fields of physics. Ultracold molecules in the micro- and nano-Kelvin regimes promise to bring powerful new capabilities to quantum emulation and quantum computing, thanks to their rich internal degrees of freedom compared to atoms. They also open new possibilities for precision measurement and the study of quantum chemistry. Quantum gases of atoms were made possible by collision-based cooling schemes, such as evaporative cooling. For ultracold molecules, thermalization and collisional cooling have not been realized. With other techniques such as supersonic jets and cryogenic buffer gases, studies have been limited to temperatures above 10 mK. Here we show cooling of NaLi molecules at micro- and nano-Kelvin temperatures through collisions with ultracold Na atoms, both prepared in their stretched hyperfine spin states. We find a lower bound on the elastic to inelastic collision ratio between molecules and atoms greater than 50 -- large enough to support sustained collisional cooling. By employing two stages of evaporation, we increase the phase-space density (PSD) of the molecules by a factor of 20, achieving temperatures as low as 220 nK. The favorable collisional properties of a Na and NaLi mixture show great promise for making deeply quantum degenerate dipolar molecules and suggest the potential for such cooling in other systems.

==> new/draft.tex <==

%\documentclass{article}
% \documentclass[prl,twocolumn]{revtex4-1}
% \usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{braket}
\usepackage{amsmath}
\usepackage{pgf}   % need for figures
\usepackage{subfig}
\usepackage{graphicx}
\usepackage{caption}
% \usepackage[justification=centering]{caption}
\captionsetup{justification=justified, singlelinecheck=false}
\usepackage{xcolor}

\graphicspath{ {./images/} }
\renewcommand{\figurename}{Fig.}
\begin{document}
	\title{Sympathetic cooling of dipolar molecules to the nanokelvin regime}
	\author{BEC3}
	\date{\today}
	
	\maketitle
	
	\section{Introduction}
	Since the original work on Bose-Einstein condensation, the field of quantum degenerate gases has grown tremendously. Ultracold gases of bosonic and fermionic atoms allow the quantum emulation of important systems from condensed matter and nuclear physics, as well as the study of novel many-body states with no analog in other fields of physics. The potential for such systems in precision measurement and quantum computing is beginning to be realized. 
	
	Ultracold molecules in the micro- and nanoKelvin regimes promise to bring powerful new capabilities to quantum emulation, quantum computing, and precision measurement. In recent years, assembling molecules from ultracold atoms and the direct laser-cooling of molecules have both expanded to new molecules and new regimes. Molecule assembly takes advantage of the powerful collisional cooling techniques of evaporative and sympathetic cooling of atoms but cannot fully capitalize on these due to inefficiencies in the molecule production process.
	
	Recent years have seen tremendous progress in the direct laser cooling of molecules. While atomic systems have demonstrated laser-cooling to quantum degeneracy, these schemes still require favorable ratios of elastic to inelastic collisions. Whether directly laser cooled or assembled from ultracold atoms, further cooling of molecules demands these favorable collision properties.
	
	As such, achieving collisional cooling of ultracold molecules is a long-standing goal of the field. Several collisional techniques can cool molecules to temperatures below $1\;{\rm K}$ including helium buffer gas cooling\cite{BufferGasCaH}, supersonic expansion\cite{Supersonic_CO}, and controlled collisions in crossed molecular beams\cite{Ar-NO_Collisions}. However, none of these techniques have been demonstrated to work below $100\;{\rm mK}$. Cooling to quantum degeneracy requires a technique that works in the micro- and nanoKelvin regimes.
	
	The desire to reach lower temperatures has motivated many searches for good collisional properties---defined as a ratio of elastic to inelastic collisions much greater than 1---in a variety of systems. Many promising systems have failed to see evidence for elastic collisions. Some evidence for elastic collisions has been seen in the OH and ${\rm O}_2$ systems at temperatures below $1\;{\rm K}$ but neither has seen definitive evidence for collisional cooling. Chemically stable molecular species assembled from ultracold atom have thus far shown anomalously high inelastic loss rates that preclude collisional cooling.
	
	In this paper we report clear evidence for sympathetic cooling of rovibrational ground-state triplet NaLi molecules by Na atoms. Sympathetic cooling of one atomic species by another has been observed in a variety of ultracold atomic mixtures but triplet NaLi is an unlikely place to find sufficiently good collisional properties. In addition to being a metastable electronic state, NaLi has energetically allowed chemical reactions, even in the electronic ground state. Furthermore, we perform our experiments in an excited hyperfine state of the rovibrational ground state. Nonetheless, we report clear thermalization and sympathetic cooling to $200\;{\rm nK}$. We observe increases of phase-space density as high as 25 times, opening the possibility of collisionally cooling to deep quantum degeneracy.
	
	\section{}
	We produce an ultracold mixture of Na and Li in their positively stretched hyperfine states (in basis $\ket{F,m_{F}}$, $\ket{2,2}$ for Na, and $\ket{3/2,3/2}$ for Li) in the Ioffe-Pritchard magnetic trap at the bias field of 2 G, by evaporatively cooling the Na atoms with RF-knife and sympathetically cooling the Li atoms with cooled Na atoms \cite{SympatheticLiCool}. Then, the mixture is transferred into the combination of two coaxial optical traps: 1064nm optical dipole trap (ODT) (30$\mu m$ waist, 10 Watt) and 1596nm 1D optical lattice (50$\mu m$ waist, 4 Watt). After 0.6 sec of forced evaporation of 1064 ODT, the sample is transferred to the lowest-energy Zeeman states   (in basis $\ket{F,m_{F}}$, $\ket{1,1}$ for Na, and $\ket{1/2,1/2}$ for Li) through the Landau-Zener magnetic field sweep, solely in the 1596nm optical lattice. In this 1596nm 1D lattice, we improve the lifetime of the NaLi molecules in the triplet ground state by suppressing the spontaneous photon scattering in molecular transitions and providing large axial confinement that sufficiently overcomes the anti-trapping curvature provided by the coils that generate high bias field \cite{NaLiGround} (Fig. something that shows loss coefficient close to the universal loss coeff.). By controlling the microwave power for the Landau-Zener sweep, we intentionally make the spin-flip imperfect and leave a fraction of Na atoms in the stretched hyperfine state as coolants for NaLi molecules. At 745.605 G which is 205 mG above an interspecies Feshbach resonance, the final mixture contains ${\sim}1.7\times10^{6}$ of Na and Li atoms in the lowest-energy Zeeman states with ${\sim}0.7\times10^6$ Na atoms in the stretched hyperfine state at the temperature of ${\sim}3 \mu K$, which corresponds to the peak density of xxx, T/$T_F$, $T/T_c$. (Any comments on trap frequencies, trap depth for atoms?) 
	
	As previously demonstrated \cite{NaLiFesh, NaLiGround}, we make $3.5\times10^{4}$ Feshbach molecules in $a^{3}\Sigma^{+}$, $v$=10, N=2, $m_{N}$=−2 state by sweeping the magnetic field across the narrow resonance at 745 G ($v$, N are the vibrational and rotational molecular quantum numbers, respectively). ${\sim}98\%$ of the Feshbach state is transferred to the triplet grounds state ($a^{3}\Sigma^{+}, v$=0, N=0) by means of $30\mu s$ long Stimulated Raman Adiabatic Passage (STIRAP) with the intermediate state ($v$=11, N= 1, $m_{N}$=−1) in $c^{3}\Sigma^{+}$ excited potential. The STIRAP frequencies (upleg: 833 nm [360.00381(1) THz], downleg: 819nm [366.23611(1) THz] \cite{NaLiPA, NaLiTwoPhoton, NaLiGround}) are obtained from two home-built external cavity diode (ECDL) lasers \cite{ECDL}, and the relative linewidth less than 1KHz is achieve by locking the lasers to an ultra-low-expansion cavity. In order to attain sufficient optical power for the upleg transition, we use a 500mW high-power diode laser which is injection-locked with the ${\sim}$2mW output of the ECDL as a seed. After the Feshbach sweep followed by STIRAP, a resonant light pulse is applied for 1 ms to clean the free atoms not being associated to molecules. Since Na atoms in the lowest-energy Zeeman state are optically pumped by the resonant light into a dark Zeeman state (which adiabatically connects to $\ket{F,m_{F}} = \ket{2,1}$ at the low bias field), full removal of free atoms is achieved by addressing the dark state with an extra frequency component added to the cleanout light. (necessary to give clean out light intensities?). Thereby, we do not need to drop the magnetic field for cleaning of the atoms at the low field like in our previous study \cite{NaLiGround}, which causes significant heating and loss of the molecules. The detection of ground state molecules is performed with the absorption imaging of the dissociated molecules, after a reverse STIRAP followed by magnetic field sweep across the Feshbach resonance. 
	
	Due to the differential polarizability from the $1596 \rm nm$ optical lattice, molecules feel deeper trapping potential than atoms do. This results in the increase of  kinetic energy associated with the center-of-mass motion and in turn, of temperature as atoms turn to molecules. Therefore, in order to measure accurate temperature of molecules, we dissociate them not in the optical trap but in free space. Subsequently, the temperature of molecules is estimated from the density profile fit of the dissociated atoms for a given time-of-flight (TOF). The ratio of the particles' trap depths is determined by the factor $(m\omega^{2})_{NaLi}/(m\omega^{2})_{Na} \sim 2.6$, $(m\omega^{2})_{NaLi}/(m\omega^{2})_{Li} \sim 2.2$, where $\omega$ is a trap frequency and $m$ is a particle mass. After STIRAP, the temperature of molecules is $2.80(5)\rm \mu K$, while the temperature of Na atoms is $2.40(4)\rm \mu K$. As molecules thermalize with Na atoms while a hot fraction of atoms evaporate out of the trap, the temperature of both particles settle to $2.25(5)\rm \mu K$ in 250 $ms$. 
	
	As shown in \figurename{\ref{fig:thermalization}} a, a thermalization rate is measured with a larger temperature difference between molecules and Na atoms, after a single evaporation. The thermalization rate from the exponential model, $T(t) = T_{0,0} e^{-t/\tau} + T_{0,1}$, is $1/\tau = 28(6) \rm (1/sec)$, while from one-body loss model, the molecule loss rate is $\gamma = 1.26(7) (1/sec)$.
	
	\begin{figure}[h]
	    \centering
		\includegraphics[width=0.5\textwidth,scale=0.7]{images/setup2.pdf}
		\caption{Experimental setup}
		\label{fig:setup2}
	\end{figure}
	
	
	% \begin{figure}[h]
	%     \centering
	%     \includegraphics[width=0.5\textwidth, scale=0.7]{images/Na_with_mol.pdf}
	%     \caption{Na}
	%     \label{fig:Na with mol}
	% \end{figure}
	
	% \begin{figure}[h]
	%     \centering
	%     \includegraphics[width=0.5\textwidth, scale=0.7]{images/Thermalization_comb_log.pdf}
	%     \caption{Thermalization log}
	%     \label{fig:thermalization log}
	% \end{figure}
	
%	\begin{figure}[h]
%		\centering
%		\includegraphics[width=0.5\textwidth, scale=0.7]{images/Thermalization_comb.pdf}
%		\caption{Thermalization}
%		\label{fig:thermalization}
%	\end{figure}
%	

	\begin{figure}[!ht]
% 		\centering
		\includegraphics[clip, width=0.5\textwidth, scale=0.7]{images/evap_seq.pdf}
		\caption{Evaporation sequence. The initial trap depth is 5 (arb. unit), and at the end of evaporation, we recompress the trap to 5 for straightfoward comparison of density. a. Single evaporation consists of $(i)$ $100ms$ exponential fored evaporation, and $(ii)$ $500ms$ recompression. b. Double evaporation consists of $(i)$ $100ms$ exponential fored evaporation, $(ii)$ $50ms$ recompression to the initial trap for fast thermalization followed by $30ms$ hold, $(3)$ $300ms$ exponential evaporation, and $(4)$ $200ms$ recompression.}
		\label{fig:evap_seq}
	\end{figure}

	\begin{figure}[!ht]
%		\subfloat{%
%			\includegraphics[clip,width=\columnwidth]{images/Thermalization_comb_break.pdf}%
%		}\\[-1ex]
%		
%		\subfloat{%
%			\includegraphics[clip,width=\columnwidth]{images/psd_avg_single_double.pdf}
%		}\\[-3ex]
%
		\includegraphics[width=0.5\textwidth, scale=0.7]{images/Thermalization_comb_break.pdf}
		\caption{Thermalization of NaLi and Na, with the evaporation sequence  \figurename{\ref{fig:evap_seq} a}. The forced exponential evaporation is performed down to trap depth of 0.5, and the trap is recompressed to 4. The molecule number and the temperature are measured at each hold time after the recompression. The dotted line is the exponential fit. }
		\label{fig:thermalization}
	\end{figure}
	
	% \begin{figure*}[h]
	%     \centering
	%     \subfigure[Evaporation sequence]{
	%     {\includegraphics[width=0.5\textwidth, scale=0.7]{images/evap_seq.pdf}}}
	%     \qquad
	%     \subfigure[PSD]{
	%     {\includegraphics[width=0.5\textwidth, scale=0.7]{images/psd_avg_single_double.pdf}}}
	%     \caption{Evaporation}
	%     \label{fig:evap}
	% \end{figure*}
	

	% \begin{figure}[h]
	%     \centering
	%     \includegraphics[width=0.5\textwidth, scale=0.7]{images/psd_single_evap.pdf}
	%     \caption{}
	%     \label{fig:psd_single evap}
	% \end{figure}
	
	% \begin{figure}[h]
	%     \centering
	%     \includegraphics[width=0.5\textwidth, scale=0.7]{images/psd_double_evap.pdf}
	%     \caption{}
	%     \label{fig:psd_double evap}
	% \end{figure}
	
	\begin{figure}[!ht]
		\includegraphics[width=0.5\textwidth, scale=0.7]{images/psd_avg_single_double.pdf}
		\caption{The comparison of single, double, and no evaporation. The x-axis is the trap depth at the end of the forced exponential evaporation ($(i)$ of the single evaporation a., and $(1)$ of the double evaporation b. in \figurename{ \ref{fig:evap_seq}}). For the double evaporation b., we evaporate down to the trap depth of 0.25 in $(3)$ in which we still have molecular signal high enough for consistent temperature estimation.}			
		\label{fig:psd_evap}
	\end{figure}
	
	\begin{figure}[!ht]
		\includegraphics[width=0.5\textwidth, scale=0.7]{images/psd_avg_single_double_with_base.pdf}
		\caption{}
		\label{fig:psd_evap}
	\end{figure}
	
%	\begin{figure}[h]
%		\centering
%		\includegraphics[width=0.5\textwidth, scale=0.7]{images/psd_avg_single_double_old.pdf}
%		\caption{Sympathetic cooling}
%		\label{fig:psd_evap}
%	\end{figure}
%	
	\begin{figure}[!ht]
		\includegraphics[width=0.5\textwidth, scale=0.7]{images/heating_avg.pdf}
		\caption{Sympathetic heating. After parametrically driving the trap depth at the frequency of $2 \times  \omega_{Na}$ (the amplitude, $20 \%$ of the trap detph, for $100ms$), we selectively heat Na atoms. After the heating, molecules thermalize to higher temperature as colliding with Na atoms.}
		\label{fig:heating}
	\end{figure}
	
	
	\section{Conclusion}
	In summary, we present the first clear evidence for collisional cooling of molecules at micro- and nanoKelvin temperatures. We find a ratio of elastic to inelastic collisions greater than 50 and observe increases in phase-space density by a factor of 25. An upgraded optical dipole trap should allow cooling into the quantum degenerate regime. Further, the atomic and molecular states used in this work are magnetically trappable. If molecules could be produced in a magnetic trap, sympathetic cooling with sodium should allow for the production of deeply degenerate quantum gases of dipolar molecules. Such gases would open new areas of inquiry in quantum emulation with long-ranged interactions and quantum computing with ultracold molecules.
	
	
	\section{Outline}
	Cold molecules for quantum chemistry, quantum simulation, quantum computation
	\begin{itemize}
		\item Degeneracy key for qsim and qcomp
	\end{itemize}
	Cooling molecules is hard
	\begin{itemize}
		\item Ultracold assembly
		\item Direct laser cooling
		\item Cooling to degeneracy requires good collisions (Florian and Vladan references) 
	\end{itemize}
	Long-standing search for collisional cooling of cold neutral molecules
	\begin{itemize}
		\item evaporative cooling of single species: OH, ${\rm O}_2$ (deal with OH issues in footnote)
		\item high loss in ultracold samples: NaRb, NaK, RbCs
	\end{itemize}
	Sympathetic cooling
	\begin{itemize}
		\item sympathetic cooling allows using good elastics and more easily cooled partner
		\item coulomb makes ions straight-forward
		\item buffer gas cooling to ~1 K    
		\item NH + N, CaH + Li, ${\rm O}_2$ + Li 
		\item ultracold sympathetic cooling of atoms (ref Weiman Rb F=2/F=1 BECs, Na/Li cooling, Li-Yb(?))
	\end{itemize}
	Triplet NaLi is an unlikely place to find good collisional properties
	\begin{itemize}
		\item Excited electronic level
		\item Upper hyperfine state
		\item chemically reactive
		\item In this paper we describe…
	\end{itemize}
	Atom preparation sequence (w Na 1 and 8 + Li 1)
	\begin{itemize}
		\item Use of imperfect transfer to set state 8 population
		\item Use of 1596nm lattice to avoid spontaneous scatter by molecules and confine axially (ref PRL)
	\end{itemize}
	Feshbach +STIRAP +blast sequence description
	\begin{itemize}
		\item Include the specific molecular levels in these steps (ref PCCPs)
		\item Ref PRL for more details
	\end{itemize}
	To understand collisions we need careful calibrations of density and temperature
	\begin{itemize}
		\item Describe differences in Na vs NaLi trap potentials
		\item Describe ToF dissociation imaging and effect on inferred temperatures
		\item Due to differing trap potentials already some cooling if you simply hold without evap
	\end{itemize}
	Holding for thermalization at various trap depths
	\begin{itemize}
		\item Describe sequence for with and without Na8 measurements
		\item Discuss evap to 1V and hold or resqueeze to 2V data 
	\end{itemize}
	Modeling to extract elastic cross-sections
	\begin{itemize}
		\item Describe the nature of the models and the results
	\end{itemize}
	Heating data
	\begin{itemize}
		\item Describe experimental sequence
		\item Describe additions to cooling model and discuss results
	\end{itemize}
	Evaporation 1
	\begin{itemize}
		\item Lifetime curves for NaLi with and without state 8
		\item Explain trade-offs between molecule-molecule loss, atom-molecule thermalization rates, and efficiency
	\end{itemize}
	Evaporation 2
	\begin{itemize}
		\item Explain phase-space density calculation	
		\item Describe experimental sequence and results
	\end{itemize}
	Prospects
	\begin{itemize}
		\item 2 sentence recapitulation
		\item Future tailoring of trap potential could allow for more optimal sequence (ref Deep’s fast BEC)
		\item Potential to magnetically trap and evaporate triplet NaLi to degeneracy
		\item Applicability to other systems (?)
		\item Opens a new era of q sim and q comp with molecules
	\end{itemize}
	
	\bibliographystyle{plain}
	\bibliography{SympCool}
	
	
\end{document}

